Data-driven Stochastic Output-Feedback Predictive Control: Recursive Feasibility through Interpolated Initial Conditions

The paper investigates data-driven output-feedback predictive control of linear systems subject to stochastic disturbances. The scheme relies on the recursive solution of a suitable data-driven reformulation of a stochastic Optimal Control Problem (OCP), which allows for forward prediction and optimization of statistical distributions of inputs and outputs. Our approach avoids the use of parametric system models. Instead it is based on previously recorded data using a recently proposed stochastic variant of Willems' fundamental lemma. The stochastic variant of the lemma is applicable to a large class of linear dynamics subject to stochastic disturbances of Gaussian and non-Gaussian nature. To ensure recursive feasibility, the initial condition of the OCP -- which consists of information about past inputs and outputs -- is considered as an extra decision variable of the OCP. We provide sufficient conditions for recursive feasibility and closed-loop practical stability of the proposed scheme as well as performance bounds. Finally, a numerical example illustrates the efficacy and closed-loop properties of the proposed scheme.

==> Resource/Sec3_ProblemStatement.tex <==

\section{Problem statement} \label{sec:problem_statement}

%\textbf{Goal}: Output-Feedback Stochastic Data-Driven Predictive control\\
%\textbf{Assumptions:} A posteriori measurable stochastic disturbance


see \cite{Berberich2021t}, for the deterministic case.

Consider the following data-driven OCP based on \eqref{eq:extended_dyna}
\begin{subequations} \label{eq:stochasticOCP}
\begin{align}
 \min_{
   \Xi\pred{\cdot}{k},U\pred{\cdot}{k},Y\pred{\cdot}{k}
    }   \sum_{i=0}^{N-1}  \mean \big[ \| Y\pred{i}{k}\|^2_Q + &\|U\pred{i}{k}\|^2_R\big] +  \mean \big[ \| Z_{N|k}\|^2_P\big]
   \hspace{1pt}  \label{eq:stochasticOCP_obj}\\
\text{s.t. } 
		\begin{bmatrix}  
	\Yf \\ \Uf \\ \Wf			
\end{bmatrix}   G &= 
\begin{bmatrix} 
	Y\pred{[0,N-l-1]}{k} \\ U\pred{[0,N-l-1]}{k}\\ W\pred{[0,N-l-1]}{k} 
\end{bmatrix}\\
		\begin{bmatrix}  
	\Yfi \\ \Ufi \\ \Wfi			
\end{bmatrix}   G &= 
\begin{bmatrix} 
	Y\pred{[-l,-1]}{k} \\ U\pred{[-l,-1]}{k}\\ W\pred{[-l,-1]}{k} 
\end{bmatrix}\\
\prob \big[Y\pred{i}{k} \relx \in  \set Y \big]\geq 1 - \varepsilon_y, &\forall i\in \I_{[k,k+N-1]}, \label{eq:chance_Y}\\
\prob \big[U\pred{i}{k} \relx \in  \set U \big]\geq 1 - \varepsilon_u, &\forall i\in \I_{[k,k+N-1]},  \label{eq:chance_U} \\
\mean \big[Z_{N|k} \big] \in  \Xf,\, \covar\big[ Z_{N|k} \big] \leq \Gamma,\,& Z_{N|k} =  \begin{bmatrix}
	\mbf{Y}_{[N-l,N-1]|k}\\
	\mbf{U}_{[N-l,N-1]|k}
\end{bmatrix} \label{eq:terminalCons}
\end{align}
\end{subequations}
%Note that this OCP obtains an initial and a terminal extended states
% \[\Xi_{\mcl{I},k} =  \begin{bmatrix}
%\bar{\mbf{Y}}_{[k-l,k-1]}\\
%\bar{\mbf{U}}_{[k-l,k-1]}\\
%\bar{\mbf{W}}_{[k-l,k-1]}
%\end{bmatrix}, \quad Z_{\mcl{T},k} =  \begin{bmatrix}
%\mbf{Y}_{[N-l,N-1]|k}\\
%\mbf{U}_{[N-l,N-1]|k}
%\end{bmatrix} .\]
\begin{assumption}
	There exist matrices $P = P^\top \succ 0$ and $K \in \R^{\dimu \times \dimz}$, and a set $\Xf$ such that for all $z\in \Xf$
	\begin{equation}\label{eq:terminal_P}
		\|(\tilde{A}+\tilde{B}K)z\|_P^2 \leq \|z\|_P^2 - \frac{1}{2} z^\top K^\top R K z - \|y|^2_Q
	\end{equation}
	\begin{equation}\label{eq:LypunovEqCov}
		(\tilde{A}+\tilde{B}K)\Gamma (\tilde{A}+\tilde{B}K)^\top -\Gamma +\widehat{\Sigma} = 0,
	\end{equation}
with $\widehat{\Sigma}$ is an upperbound on $\tilde{E}\covar[\mbf{W}_{[k-l,k-1]}]\tilde{E}^\top$.

\end{assumption}



%\subsection{Data-driven stochastic OCP via PCE}


Causality condition


Given the PCE coefficients of the current state $\pce[j]{x}_k$ and future process noise $\pce[j]{w}_{k+i}$,  $i \in \I_{[0,N-1]}$, $j\in \I_{[0,L-1]}$, we have
\begin{subequations}\label{eq:stochOCP_PCE}
	\begin{gather}
		\min_{\substack{
				\pce{g}^{\cdot}, \pce{y}^{\cdot}\pred{\cdot}{k}, \\
				\pce{u}^{\cdot}\pred{\cdot}{k}, \pce{$\xi$}^{\cdot}_{\mcl{T},k}
		}    }
		\sum_{j=0}^L \bigg(\sum_{i=0}^{N-1} \Big(\| \pce[j]{y} \pred{i}{k}\|^2_Q  +\|\pce[j]{u}\pred{i}{k}\|^2_R\Big) + \|\pce[j]{z}_{N|k}\|_P^2 \bigg) \langle\phi^{j}\rangle^2 \\
		\text{s.t.} \quad \forall j\in \I_{[0,L-1]},  \, \forall i \in \I_{[0,N-1]} \nonumber \\
			\begin{bmatrix}  
		\Yfi \\ \Ufi \\ \Wfi			
	\end{bmatrix}  \pce[j]{g} = 
	\begin{bmatrix} 
		\pce[j]{y}\pred{[-l,-1]}{k} \\ \pce[j]{u}\pred{[-l,-1]}{k}\\ \pce[j]{w}\pred{[-l,-1]}{k} 
	\end{bmatrix}\\ 
		\begin{bmatrix} 
	\Yf \\ \Uf \\ \Wf			
\end{bmatrix}   \pce[j]{g} = 
\begin{bmatrix}
	\pce[j]{y}\pred{[0,N-l-1]}{k} \\ \pce[j]{u}\pred{[0,N-l-1]}{k}\\ \pce[j]{w}\pred{[0,N-l-1]}{k} 
\end{bmatrix} \label{eq:stochOCP_Hankel_pce} \\
		\pce[0]{y}\pred{i}{k}  \pm  \sigma(\varepsilon_y) \sqrt{\sum_{j'=1}^{L-1} (\pce[j']{y}\pred{i}{k})^2  \langle\phi^{j'}\rangle^2 } \in  \set Y, \label{eq:chance_Y_PCE}\\
		\pce[0]{u}\pred{i}{k}  \pm  \sigma(\varepsilon_u) \sqrt{\sum_{j'=1}^{L-1} {(\pce[j']{u}\pred{i}{k}})^2  \langle\phi^{j'}\rangle^2  } \in \set U,  \label{eq:chance_U_PCE}\\
		\pce[0]{z}_{N|k} \in  \Xf, \quad \sum_{j=1}^{L-1} \pcecoe{z}{j}_{N|k} \pcecoe{z}{j\top}_{N|k} \langle\phi^{j}\rangle^2\leq \Gamma,    \quad \pce[j]{z}_{N|k} =  \begin{bmatrix}
				\pce[j]{y}_{[N-l,N-1]|k}\\
				\pce[j]{u}_{[N-l,N-1]|k}
		\end{bmatrix}    \label{eq:PCE_Xf}\\ 
		\edit{	\pce{u}\pred{i}{k}^{j'} = 0,  \forall j'\in \I_{[L_{\xi}+iL_w+1,L]}.} \label{eq:causality}
	\end{gather}
\end{subequations}

\textbf{Research Questions}
\begin{itemize}
\item How to determine the terminal ingredients in a data-driven fashion? 
\item How to design a predictive control algorithm with recursive feasibility and stability guarantees?
\end{itemize}

